SoulX-LiveAct: Towards Hour-Scale Real-Time Human Animation with Neighbor Forcing and ConvKV Memory

Autoregressive (AR) diffusion models offer a promising framework for sequential generation tasks such as video synthesis by combining diffusion modeling with causal inference. Although they support streaming generation, existing AR diffusion methods struggle to scale efficiently. In this paper, we identify two key challenges in hour-scale real-time human animation. First, most forcing strategies propagate sample-level representations with mismatched diffusion states, causing inconsistent learning signals and unstable convergence. Second, historical representations grow unbounded and lack structure, preventing effective reuse of cached states and severely limiting inference efficiency. To address these challenges, we propose Neighbor Forcing, a diffusion-step-consistent AR formulation that propagates temporally adjacent frames as latent neighbors under the same noise condition. This design provides a distribution-aligned and stable learning signal while preserving drifting throughout the AR chain. Building upon this, we introduce a structured ConvKV memory mechanism that compresses the keys and values in causal attention into a fixed-length representation, enabling constant-memory inference and truly infinite video generation without relying on short-term motion-frame memory. Extensive experiments demonstrate that our approach significantly improves training convergence, hour-scale generation quality, and inference efficiency compared to existing AR diffusion methods. Numerically, LiveAct enables hour-scale real-time human animation and supports 20 FPS real-time streaming inference on as few as two NVIDIA H100 or H200 GPUs. Quantitative results demonstrate that our method attains state-of-the-art performance in lip-sync accuracy, human animation quality, and emotional expressiveness, with the lowest inference cost.

==> content/0.abstract.tex <==
\begin{abstract}
\end{abstract}




==> content/5.Contribution.tex <==
\section{Project Contributions}
All contributors are listed in no particular order.
\begin{itemize}
\item \textbf{Project Sponsor:} Ming Tao, Shunshun Yin
\item \textbf{Project Leader:} Siyuan Liu
\item \textbf{Algorithm:} Le Shen, Qian Qiao, Tan Yu
\item \textbf{Deployment \& Acceleration:} Ke Zhou, Tianhang Yu, Yu Zhan
\item \textbf{Data \& Evaluation:} Tan Yu, Tianhang Yu, Dingcheng Zhen
\end{itemize}



==> content/6.Statement.tex <==
\section{Ethics Statement}
% 本研究旨在推动高保真数字人技术在正向场景中的应用。我们郑重声明，本研究中使用的所有训练与测试数据均来源于公开可访问的学术数据集。论文及附录中展示的所有可视化结果均为模型合成生成的数字内容，不包含任何真实个体的非公开个人隐私信息（PII）。

%我们充分意识到高保真视频生成技术具有双重用途（Dual-use）的性质，存在被滥用于制造深度伪造（Deepfakes）或传播虚假信息的潜在风险。我们坚决反对任何形式的技术滥用，并倡导“负责任的 AI”开发原则。为此，我们支持并呼吁社区开发更先进的伪造检测算法及不可见水印技术，以提升生成内容的透明度与可追溯性。我们将持续关注技术发展的伦理边界，确保研究成果服务于社会公共利益。

This research aims to advance digital human synthesis for beneficial applications. We confirm that all datasets utilized in this study are derived from publicly accessible academic repositories. The visual demonstrations presented in this report are fully synthetic and do not contain the Personally Identifiable Information (PII) of private individuals.

We acknowledge the dual-use nature of high-fidelity video generation technology and the potential risks associated with its misuse, such as the creation of deepfakes or the spread of misinformation. We firmly condemn any malicious application of this technology and advocate for the principles of Responsible AI. To mitigate these risks, we support the development of robust forgery detection algorithms and the implementation of invisible watermarking mechanisms to ensure content transparency and traceability. We remain committed to adhering to ethical guidelines and ensuring that our contributions promote the safe and positive evolution of the field.
